FusionSF: Fuse Heterogeneous Modalities in a Vector Quantized Framework for Robust Solar Power Forecasting

Accurate solar power forecasting is crucial to integrate photovoltaic plants into the electric grid, schedule and secure the power grid safety. This problem becomes more demanding for those newly installed solar plants which lack sufficient data. Current research predominantly relies on historical solar power data or numerical weather prediction in a single-modality format, ignoring the complementary information provided in different modalities. In this paper, we propose a multi-modality fusion framework to integrate historical power data, numerical weather prediction, and satellite images, significantly improving forecast performance. We introduce a vector quantized framework that aligns modalities with varying information densities, striking a balance between integrating sufficient information and averting model overfitting. Our framework demonstrates strong zero-shot forecasting capability, which is especially useful for those newly installed plants. Moreover, we collect and release a multi-modal solar power (MMSP) dataset from real-world plants to further promote the research of multi-modal solar forecasting algorithms. Our extensive experiments show that our model not only operates with robustness but also boosts accuracy in both zero-shot forecasting and scenarios rich with training data, surpassing leading models. We have incorporated it into our eForecaster platform and deployed it for more than 300 solar plants with a capacity of over 15GW.

==> tables/3_zeroshot.tex <==
\begin{table}[t]
\centering
\caption{The performance of zero-shot learning on MMSP dataset, using various range of plants for training and testing on plants \#0-\#9.}
% \vskip 0.15in
\begin{center}
\begin{small}
% \scalebox{1.00}{
% \begin{sc}
\begin{tabular}{c|cccccc}
\toprule

% \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Size} & \multicolumn{2}{c|}{Seq. Len.} & Spatial Resolution \\
% & train & val & test & in & out & H $\times$ W  \\

\multirow{2}{*}{Setting}  & \multicolumn{2}{c}{All} & \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Hard} \\
% \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} 
% Models                     & mae     & rmse    &  &  & \\
% Setting & MAE & RMSE & easy mae & easy rmse & hard mae & hard rmse \\ % mae & rmse & mae & rmse \\
 & MAE & RMSE & mae & rmse & mae & rmse \\ % mae & rmse & mae & rmse \\

\midrule

3modal          & 0.04124 & 0.09222 & 0.03891 & 0.08359 & 0.04980 & 0.10690 \\
10-20 train & 0.04287 & 0.09188 & 0.05351 & 0.08067	& 0.04078 & 0.10624 \\
10-30 train & 0.04122 & 0.08889 & 0.05002 & 0.08056 & 0.03752 & 0.10672 \\
10-40 train & 0.04076 & 0.08764 & 0.05002 & 0.07906 & 0.03701 & 0.10588 \\
10-60 train & 0.04072 & 0.08647 & 0.05008 & 0.07737 & 0.03692 & 0.10566 \\


% Crossvivit 2modal (ts+context) & 0.05789 &	0.11818 \\ %& 0.04891 & 0.09924 & 0.08007 & 0.15535 \\
% Crossvivit 2modal (ts+nwp)     &  0.04503  & 0.09890  \\%&  &  & \\
% Crossvivit 3modal          & 0.04124 & 0.09222 \\ %& 0.03891 & 0.08359 & 0.04980 & 0.10690 \\
% Crossvivit 3modal zeroshot & 0.04287 & 0.09188 &  &  & \\
% Crossvivit 3modal zeroshot 30site train & 0.04076 & 0.08764 &  &  & \\
% Crossvivit 3modal zeroshot 50site train & 0.04072 & 0.08647 &  &  & \\

\bottomrule
\end{tabular}
\label{tab3:zeroshot}

% \end{sc}
\end{small}
\end{center}
% \vskip -0.1in
%\vspace{-5mm}
\end{table}






==> tables/4_compare_era.tex <==
\begin{table}[t]
\centering
\caption{Analysis of Forecasting Error Due to NWP Inaccuracy. An Assessment using ERA5 data as ideal weather reports and Satellite(Real) observations for actual cloud conditions, with SolarTCN serving as the backbone.}
% \vskip 0.15in
\begin{center}
\begin{small}
% \scalebox{1.00}{
% \begin{sc}
\begin{tabular}{c|ccccccc}
\toprule

% \multirow{2}{*}{Models}  & \multicolumn{2}{c}{All (25210)} \\ % & \multicolumn{2}{c}{Easy (18014)} & \multicolumn{2}{c}{Hard (7196)} \\
% \cmidrule{2-3} \cmidrule{4-5} \cmidrule{6-7} 
% Models                     & mae     & rmse    &  &  & \\
Methods & Data & MAE & RMSE & \\ % mae & rmse & mae & rmse \\
\midrule
% \multirow{2}{*}{\parbox{1.2cm}{Ablation \\ of data}}  \\ %& 0.04891 & 0.09924 & 0.08007 & 0.15535 \\
% & \#2 TS+NWP     &  0.04503  & 0.09890  \\%&  &  & \\

% \midrule
Ours & TS+NWP+Satellite   & 0.04124 & 0.09222 \\
\midrule
 % & \#4 TS+NWP+Context(4 channels)   & 0.04163 & 0.09279 \\
 % & \#5 TS+NWP+Context(25km)   & 0.04144 & 0.09046 \\
 % & \#6 TS+NWP+Context(10km)   & 0.04267 & 0.08862 \\

\multirow{5}{*}{\parbox{1.2cm}{SolarTCN \\ backbone}} & NWP & 0.04443 & 0.0892921 \\

& ERA5 & 0.04222 & 0.08483 \\

\cmidrule{2-5}

& Satellite(Real) & 0.05016 & 0.10128\\

& NWP+Satellite(Real) & 0.04059 & 0.08407 \\

%   &  NWP+Satellite(Real) x4 & 0.03989 & 0.08404 \\


& ERA5+Satellite(Real) & 0.03985 & 0.08275 \\


 
% \midrule

% \multirow{5}{*}{\parbox{1.2cm}{Ablation \\ of module}} & w/o VQ & 0.4124 & 0.09222 \\ %& 0.04891 & 0.09924 & 0.08007 & 0.15535 \\
% & w/ VQ only on context & 0.04289 & 0.08875 \\
% & w/ VQ only on TS & 0.04266 & 0.09213 \\
% & w/ VQ on context\&TS\&NWP & 0.04152 & 0.08985 \\
% & Ours: w/ VQ on context\&TS & 0.04020 & 0.08881 \\
% & attention on THW & 0.03958 & 0.08636 \\
% & w/o ROPE \\
% & w/o random masking \\
% & Shared MLP & 0.04272 & 0.09462 \\

\bottomrule
\end{tabular}
\label{tab4:compare_era}

% \end{sc}
\end{small}
\end{center}
\vskip -0.2in
%\vspace{-5mm}
\end{table}


==> tables/demo.tex <==
\begin{table}[h]
\caption{Details of ETT benchmark datasets.}
\label{tab:dataset}
%\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{l|cccr}
\toprule
% Dataset & num & dim & freq \\
Dataset & Length & Dimension & Frequency \\
\midrule
ETTm1/m2 & 69680$\approx$2 years & 7 & 15 min\\
Electricity & 26304$\approx$3 years & 321 & 1h & \\
Traffic & 17544$\approx$2 years & 862 & 1h & \\
Weather & 52696$\approx$1 years & 21 & 10 min & \\
Illness & 966$\approx$18 years & 7 & 7 days\\
Exchange & 7588$\approx$20 years & 8 & 1 day\\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.3in
\end{table}
